Symmetry and reactivity of $\pi$-systems in electric and magnetic fields: a perspective from conceptual DFT

[Abridged] The extension of conceptual DFT to include external fields in chemical systems is utilised to investigate the effects of strong magnetic fields on the electronic charge distribution and its consequences on the reactivity of $\pi$-systems. Formaldehyde, H$_2$CO, is considered as a prototypical example and current-DFT calculations are used to evaluate the electric dipole moment together with the electron density and the Fukui functions, which provide insight into how H$_2$CO behaves chemically in a magnetic field. In particular, the symmetries of these quantities are analysed based on group, representation, and corepresentation theories using QSym$^2$. This allows us to leverage the simple symmetry constraints on the macroscopic electric dipole moments to make profound predictions on the more nuanced symmetry transformation properties of the microscopic frontier MOs, electron densities, and Fukui functions. This is especially useful for complex-valued MOs in magnetic fields whose detailed symmetry analyses lead us to define the new concepts of modular and phasal symmetry breaking. Through these, the connection between the vanishing constraints on the electric dipole moments and the symmetry of electron densities and Fukui functions can be formalised, and the inability of the magnetic field in all three orientations considered to induce asymmetry with respect to the molecular plane can be understood from a molecular perspective. Furthermore, the detailed forms of the Fukui functions reveal remarkable reversals in the direction of the C=O dipole moment in the presence of a parallel or perpendicular magnetic field, which can be attributed to the mixing between frontier MOs due to their subduced symmetries in magnetic fields. The findings in this work are also discussed in the wider context of a long-standing debate on the possibility to create enantioselectivity by external fields.

==> suppinfo/anionden/anionden.tex <==
\section{Electron densities of \ce{[H2CO]-} anion and density difference plots}

%  \subsection{Contour plots for the electron densities of \ce{[H2CO]-}}

    \begin{figure*}[h!]
      \centering
      \includegraphics[width=.95\linewidth]{figures/tikz/anion_densities/anion_densities.tikz.pdf}
      \caption{%
        Contour plots of the electron density $\rho(\mathbf{r})$ of the \ce{[H2CO]-} anion in various external-field configurations.
        Above each plot are the three-dimensional isosurface of the corresponding electron density at isovalue $\rho(\mathbf{r}) = 0.01$ and the representations spanned by $\rho(\mathbf{r})$ and its symmetry partners in various groups as determined by \qsymsq{} (see also Appendix~B in the main text for relevant character tables).
        Magnetic symmetries in $\mathcal{M}$ are given in terms of its  irreducible representations since electron densities are real-valued (\textit{cf.} Section~2.3.3.2 in the main text).
        All electron densities were calculated at the r\textsuperscript{2}SCAN0/cc-pVTZ level.
        The electric field strength $\mathcal{E}$ is set at \SI{0.1}{\atomicunit} and the magnetic field strength $B$ at $1.0 B_0$.
      }
      \label{fig:anion_densities}
    \end{figure*}

  \clearpage
%  \subsection{Contour plots for the electron densities of \ce{[H2CO]-}}

    \begin{figure*}[h!]
      \centering
      \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[height=.8\textheight]{figures/tikz/dendiff/dendiff_e.tikz.pdf}
        \caption*{(continued next page)}
      \end{subfigure}
    \end{figure*}

    \begin{figure*}[h!]
      \ContinuedFloat
      \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[height=.8\textheight]{figures/tikz/dendiff/dendiff_b.tikz.pdf}
      \end{subfigure}
      \caption{%
        Density difference plots in various external-field configurations.
        Each plot shows the difference $\rho(\mathbf{r}) - \rho_0(\mathbf{r})$ in the vertical \ce{C=O} plane with $\rho(\mathbf{r})$ the density of either the neutral species or the anionic one in the given field, and $\rho_0(\mathbf{r})$ the corresponding density at zero field.
        Each plot is also accompanied by an isosurface of the density difference shown at $\lvert \rho(\mathbf{r}) - \rho_0(\mathbf{r}) \rvert = 0.005$.
      }
      \label{fig:dendiff}
    \end{figure*}

==> suppinfo/hfco/hfco.tex <==
\section{Analysis results for \ce{HFCO}}

  \begin{figure}[h!]
    \centering
    \includegraphics[width=.5\linewidth]{figures/tikz/mol/mol.tikz.pdf}
    \caption{%
      Geometrical arrangement of \ce{HFCO} in all calculations.
      The molecule lies in the $yz$-plane with the \ce{C=O} bond aligning with the $z$-axis.
      \ce{H}: grey, \ce{C}: blue, \ce{O}: red, \ce{F}: orange.
    }
    \label{fig:mol}
  \end{figure}

  \subsection{Symmetry constraints on electric dipole moments}

    \begin{table}[h!]
      \centering
      \caption{%
        Symmetry groups and allowed electric dipole components $\bm{\mu}$ of \ce{HFCO} in external electric or magnetic fields.
        The allowed electric dipole components are those that are not constrained to vanish by the corresponding symmetry group.
        The geometrical arrangement of the \ce{HFCO} molecule is given in Figure~\ref{fig:mol}.
        $\mathcal{G}$ gives the unitary symmetry group of the molecule-plus-field system and $\mathcal{M}$ the magnetic symmetry group (\textit{cf.} Section~2.2.1 in the main text).
        In the absence of an external magnetic field, $\mathcal{M}$ is a grey group as denoted by the dash [Equation~(24) in the main text].
        Character tables for all groups as generated by \qsymsq{} are given in Appendix~B in the main text.
        Note that in the $\mathbf{B} = B\hat{\mathbf{x}}$ case, the system has no magnetic group due to the lack of time-reversed symmetry operations.
      }
      \label{tab:dipsym-hfco}
      \renewcommand\arraystretch{1.25}
      \begin{tabular}{%
        l |%
        M{1.9cm} M{1.9cm} |%
        M{1.9cm} M{1.9cm}
      }
        \toprule
        Field % Field
        %
        % G
        & $\mathcal{G}$ % G
        & Allowed $\bm{\mu}$ % Dipole components (G)
        %
        % M
        & $\mathcal{M}$ % M
        & Allowed $\bm{\mu}$ % Dipole components (M)
        \\
        \midrule
        % ----------
        % Zero field
        % ----------
        $\mathbf{0}$ % Field
        %
        % G
        & $\mathcal{C}_{s}(yz)$ % G
        & $\mu_y, \mu_z$ % Dipole components (G)
        %
        % M
        & $\mathcal{C}'_{s}(yz)$ % Dipole components (M)
        & $\mu_y, \mu_z$ % M
        \\[8pt]
        % --
        % Ex
        % --
        $\boldsymbol{\mathcal{E}} = \mathcal{E}\hat{\mathbf{x}}$ % Field
        %
        % G
        & $\mathcal{C}_{1}$ % G
        & $\mu_x, \mu_y, \mu_z$ % Dipole components (G)
        %
        % M
        & $\mathcal{C}'_{1}$ % M
        & $\mu_x, \mu_y, \mu_z$ % Dipole components (M)
        \\[-5pt]
        {\scriptsize (perpendicular)} &&&&
        \\
        % --
        % Ey
        % --
        $\boldsymbol{\mathcal{E}} = \mathcal{E}\hat{\mathbf{y}}$ % Field
        %
        % G
        & $\mathcal{C}_{s}(yz)$ % G
        & $\mu_y, \mu_z$ % Dipole components (G)
        %
        % M
        & $\mathcal{C}'_{s}(yz)$ % M
        & $\mu_y, \mu_z$ % Dipole components (M)
        \\[-5pt]
        {\scriptsize (in-plane)} &&&&
        \\
        % --
        % Ez
        % --
        $\boldsymbol{\mathcal{E}} = \mathcal{E}\hat{\mathbf{z}}$ % Field
        %
        % G
        & $\mathcal{C}_{s}(yz)$ % G
        & $\mu_y, \mu_z$ % Dipole components (G)
        %
        % M
        & $\mathcal{C}'_{s}(yz)$ % M
        & $\mu_y, \mu_z$ % Dipole components (M)
        \\[-5pt]
        {\scriptsize (parallel)} &&&&
        \\[8pt]
        % --
        % Bx
        % --
        $\mathbf{B} = B\hat{\mathbf{x}}$ % Field
        %
        % G
        & $\mathcal{C}_{s}(yz)$ % G
        & $\mu_y, \mu_z$ % Dipole components (G)
        %
        % M
        & - % M
        & - % Dipole components (M)
        \\[-5pt]
        {\scriptsize (perpendicular)} &&&&
        \\
        % --
        % By
        % --
        $\mathbf{B} = B\hat{\mathbf{y}}$ % Field
        %
        % G
        & $\mathcal{C}_{1}$ % G
        & $\textcolor{red}{\mu_x}, \mu_y, \mu_z$ % Dipole components (G)
        %
        % Dipole
        & $\mathcal{C}_s(yz)(\mathcal{C}_1)$ % M
        & $\mu_y, \mu_z$ % Dipole components (M)
        \\[-5pt]
        {\scriptsize (in-plane)} &&&&
        \\
        % --
        % Bz
        % --
        $\mathbf{B} = B\hat{\mathbf{z}}$ % Field
        %
        % G
        & $\mathcal{C}_{1}$ % G
        & $\textcolor{red}{\mu_x}, \mu_y, \mu_z$ % Dipole components (G)
        %
        % M
        & $\mathcal{C}_s(yz)(\mathcal{C}_1)$ % M
        & $\mu_y, \mu_z$ % Dipole components (M)
        \\[-5pt]
        {\scriptsize (parallel)} &&&&
        \\
        \bottomrule
      \end{tabular}
    \end{table}


  \subsection{Calculated electric dipole moments}

    \begin{table*}[h!]
      \centering
      \caption{%
        Electric dipole moment components (in atomic units) for \ce{HFCO} calculated using the r\textsuperscript{2}SCAN0 and cTPSS exchange-correlation functionals in 6-31G** and cc-pVTZ basis sets.
        The electric field strength $\mathcal{E}$ is set at \SI{0.1}{\atomicunit} and the magnetic field strength $B$ at \num{1.0} $B_0$.
      }
      \label{tab:dipval-hfco}
      \renewcommand\arraystretch{1.10}
      \captionsetup[subtable]{justification=centering}
      \begin{subtable}{\textwidth}
        \centering
        \subcaption{r\textsuperscript{2}SCAN0}
        \resizebox{\textwidth}{!}{
          \begin{tabular}{%
            l |%
            S[table-format=+1.9, table-alignment-mode=format, retain-explicit-plus]
            S[table-format=+1.9, table-alignment-mode=format, retain-explicit-plus]
            S[table-format=+1.9, table-alignment-mode=format, retain-explicit-plus] |%
            S[table-format=+1.9, table-alignment-mode=format, retain-explicit-plus]
            S[table-format=+1.9, table-alignment-mode=format, retain-explicit-plus]
            S[table-format=+1.9, table-alignment-mode=format, retain-explicit-plus]
          }
            \toprule
            \multirow{2}{*}{Field} % Field
            %
            & \multicolumn{3}{c|}{6-31G**}
            %
            & \multicolumn{3}{c}{cc-pVTZ}
            \\
            %
            & $\mu_x$ % mu_x 6-31G**
            & $\mu_y$ % mu_y 6-31G**
            & $\mu_z$ % mu_z 6-31G**
            %
            & $\mu_x$ % mu_x cc-pVTZ
            & $\mu_y$ % mu_y cc-pVTZ
            & $\mu_z$ % mu_z cc-pVTZ
            \\
            \midrule
            % ----------
            % Zero field
            % ----------
            $\mathbf{0}$ % Field
            %
            & 0.000000000 % mu_x 6-31G**
            & -0.504153451 % mu_y 6-31G**
            & -0.667099400 % mu_z 6-31G**
            %
            & 0.000000000 % mu_x cc-pVTZ
            & -0.539087871 % mu_y cc-pVTZ
            & -0.656739980 % mu_z cc-pVTZ
            \\[8pt]
            % --
            % Ex
            % --
            $\boldsymbol{\mathcal{E}} = \mathcal{E}\hat{\mathbf{x}}$ % Field
            %
            & +0.843025900 % mu_x 6-31G**
            & -0.510258110 % mu_y 6-31G**
            & -0.651623250 % mu_z 6-31G**
            %
            & +1.102638225 % mu_x cc-pVTZ
            & -0.529875366 % mu_y cc-pVTZ
            & -0.632962909 % mu_z cc-pVTZ
            \\[-5pt]
            {\scriptsize (perpendicular)} &&&&
            \\
            % --
            % Ey
            % --
            $\boldsymbol{\mathcal{E}} = \mathcal{E}\hat{\mathbf{y}}$ % Field
            %
            & 0.000000000 % mu_x 6-31G**
            & +1.071912414 % mu_y 6-31G**
            & -0.657722470 % mu_z 6-31G**
            %
            & 0.000000000 % mu_x cc-pVTZ
            & +1.480133793 % mu_y cc-pVTZ
            & -0.514399955 % mu_z cc-pVTZ
            \\[-5pt]
            {\scriptsize (in-plane)} &&&&
            \\
            % --
            % Ez
            % --
            $\boldsymbol{\mathcal{E}} = \mathcal{E}\hat{\mathbf{z}}$ % Field
            %
            & 0.000000000 % mu_x 6-31G**
            & -0.465176676 % mu_y 6-31G**
            & +1.280146850 % mu_z 6-31G**
            %
            & 0.000000000 % mu_x cc-pVTZ
            & -0.385131630 % mu_y cc-pVTZ
            & +1.677359970 % mu_z cc-pVTZ
            \\[-5pt]
            {\scriptsize (parallel)} &&&&
            \\[8pt]
            % --
            % Bx
            % --
            $\mathbf{B} = B\hat{\mathbf{x}}$ % Field
            %
            & 0.000000000 % mu_x 6-31G**
            & +0.827268771 % mu_y 6-31G**
            & -0.695147257 % mu_z 6-31G**
            %
            & 0.000000000 % mu_x cc-pVTZ
            & +0.709136583 % mu_y cc-pVTZ
            & -0.656474226 % mu_z cc-pVTZ
            \\[-5pt]
            {\scriptsize (perpendicular)} &&&&
            \\
            % --
            % By
            % --
            $\mathbf{B} = B\hat{\mathbf{y}}$ % Field
            %
            & 0.000000000 % mu_x 6-31G**
            & +0.528252893 % mu_y 6-31G**
            & -0.696304097 % mu_z 6-31G**
            %
            & 0.000000000 % mu_x cc-pVTZ
            & +0.690315439 % mu_y cc-pVTZ
            & -0.620750521 % mu_z cc-pVTZ
            \\[-5pt]
            {\scriptsize (in-plane)} &&&&
            \\
            % --
            % Bz
            % --
            $\mathbf{B} = B\hat{\mathbf{z}}$ % Field
            %
            & 0.000000000 % mu_x 6-31G**
            & +0.858643144 % mu_y 6-31G**
            & +1.496848359 % mu_z 6-31G**
            %
            & 0.000000000 % mu_x cc-pVTZ
            & +1.027873856 % mu_y cc-pVTZ
            & +0.732919497 % mu_z cc-pVTZ
            \\[-5pt]
            {\scriptsize (parallel)} &&&&
            \\
            \bottomrule
          \end{tabular}
        }
      \end{subtable}

      \vspace{0.5cm}

      % -----
      % cTPSS
      % -----
      \begin{subtable}{\textwidth}
        \centering
        \subcaption{cTPSS}
        \resizebox{\textwidth}{!}{
          \begin{tabular}{%
            l |%
            S[table-format=+1.9, table-alignment-mode=format, retain-explicit-plus]
            S[table-format=+1.9, table-alignment-mode=format, retain-explicit-plus]
            S[table-format=+1.9, table-alignment-mode=format, retain-explicit-plus] |%
            S[table-format=+1.9, table-alignment-mode=format, retain-explicit-plus]
            S[table-format=+1.9, table-alignment-mode=format, retain-explicit-plus]
            S[table-format=+1.9, table-alignment-mode=format, retain-explicit-plus]
          }
            \toprule
            \multirow{2}{*}{Field} % Field
            %
            & \multicolumn{3}{c|}{6-31G**}
            %
            & \multicolumn{3}{c}{cc-pVTZ}
            \\
            %
            & $\mu_x$ % mu_x 6-31G**
            & $\mu_y$ % mu_y 6-31G**
            & $\mu_z$ % mu_z 6-31G**
            %
            & $\mu_x$ % mu_x cc-pVTZ
            & $\mu_y$ % mu_y cc-pVTZ
            & $\mu_z$ % mu_z cc-pVTZ
            \\
            \midrule
            % ----------
            % Zero field
            % ----------
            $\mathbf{0}$ % Field
            %
            & 0.000000000 % mu_x 6-31G**
            & -0.441160192 % mu_y 6-31G**
            & -0.623589127 % mu_z 6-31G**
            & 0.000000000 % mu_x cc-pVTZ
            & -0.484270157 % mu_y cc-pVTZ
            & -0.610392342 % mu_z cc-pVTZ
            \\[8pt]
            % --
            % Ex
            % --
            $\boldsymbol{\mathcal{E}} = \mathcal{E}\hat{\mathbf{x}}$ % Field
            %
            & +0.861566295 % mu_x 6-31G**
            & -0.445529227 % mu_y 6-31G**
            & -0.610584021 % mu_z 6-31G**
            %
            & +1.137158616 % mu_x cc-pVTZ
            & -0.473134059 % mu_y cc-pVTZ
            & -0.588167436 % mu_z cc-pVTZ
            \\[-5pt]
            {\scriptsize (perpendicular)} &&&&
            \\
            % --
            % Ey
            % --
            $\boldsymbol{\mathcal{E}} = \mathcal{E}\hat{\mathbf{y}}$ % Field
            %
            & 0.000000000 % mu_x 6-31G**
            & +1.244473360 % mu_y 6-31G**
            & -0.602723699 % mu_z 6-31G**
            %
            & 0.000000000 % mu_x cc-pVTZ
            & +1.805587942 % mu_y cc-pVTZ
            & -0.364885680 % mu_z cc-pVTZ
            \\[-5pt]
            {\scriptsize (in-plane)} &&&&
            \\
            % --
            % Ez
            % --
            $\boldsymbol{\mathcal{E}} = \mathcal{E}\hat{\mathbf{z}}$ % Field
            %
            & 0.000000000 % mu_x 6-31G**
            & -0.389846305 % mu_y 6-31G**
            & +1.387953299 % mu_z 6-31G**
            %
            & 0.000000000 % mu_x cc-pVTZ
            & -0.239660695 % mu_y cc-pVTZ
            & +1.911552802 % mu_z cc-pVTZ
            \\[-5pt]
            {\scriptsize (parallel)} &&&&
            \\[8pt]
            % --
            % Bx
            % --
            $\mathbf{B} = B\hat{\mathbf{x}}$ % Field
            %
            & 0.000000000 % mu_x 6-31G**
            & +0.559299281 % mu_y 6-31G**
            & -0.306997213 % mu_z 6-31G**
            %
            & 0.000000000 % mu_x cc-pVTZ
            & +0.606192147 % mu_y cc-pVTZ
            & -0.239076175 % mu_z cc-pVTZ
            \\[-5pt]
            {\scriptsize (perpendicular)} &&&&
            \\
            % --
            % By
            % --
            $\mathbf{B} = B\hat{\mathbf{y}}$ % Field
            %
            & 0.000000000 % mu_x 6-31G**
            & +0.526191952 % mu_y 6-31G**
            & -0.682964369 % mu_z 6-31G**
            %
            & 0.000000000 % mu_x cc-pVTZ
            & +0.669392535 % mu_y cc-pVTZ
            & -0.578657826 % mu_z cc-pVTZ
            \\[-5pt]
            {\scriptsize (in-plane)} &&&&
            \\
            % --
            % Bz
            % --
            $\mathbf{B} = B\hat{\mathbf{z}}$ % Field
            %
            & 0.000000000 % mu_x 6-31G**
            & +0.718812883 % mu_y 6-31G**
            & +1.276925684 % mu_z 6-31G**
            %
            & 0.000000000 % mu_x cc-pVTZ
            & +0.879825148 % mu_y cc-pVTZ
            & +0.798810909 % mu_z cc-pVTZ
            \\[-5pt]
            {\scriptsize (parallel)} &&&&
            \\
            \bottomrule
          \end{tabular}
        }
      \end{subtable}
    \end{table*}

    \pagebreak

  \subsection{Fukui functions}

      \begin{figure*}[h!]
        \centering
        \includegraphics[width=\linewidth]{figures/tikz/fukui/fukui.tikz.pdf}
        \caption{%
          Contour plots of the Fukui function for nucleophilic attack, $f^+(\mathbf{r})$, of \ce{HFCO} in various external-field configurations.
          Above each plot are the three-dimensional isosurface of the corresponding Fukui function at isovalue $f^+(\mathbf{r}) = 0.01$ and the representations spanned by $f^+(\mathbf{r})$ and its symmetry partners in various groups as determined by \qsymsq{} (see also Appendix~B in the main text for relevant character tables).
          Magnetic symmetries in $\mathcal{M}$ are given in terms of its  irreducible representations since Fukui functions are real-valued (\textit{cf.} Section~2.3.3.2 in the main text).
          Positive regions (blue) indicate sites in the system that are favourable for nucleophilic attack.
          All Fukui functions were calculated using the finite-difference approach [Equation~(22) in the main text] at the r\textsuperscript{2}SCAN0/cc-pVTZ level.
          The electric field strength $\mathcal{E}$ is set at \SI{0.1}{\atomicunit} and the magnetic field strength $B$ at $1.0 B_0$.
        }
        \label{fig:fukui-hfco}
      \end{figure*}

==> suppinfo/preamble.tex <==
% ========
% Preamble
% ========



% ------------------
% Scientific support
% ------------------
% Chemistry
\usepackage[version=4]{mhchem}

% Scientific typesetting
\usepackage{siunitx}
\DeclareSIUnit{\atomicunit}{a.u.}
\DeclareSIUnit\atomicmassunit{u}
\DeclareSIUnit\angstrom{\text {Å}}

% -------------
% Maths support
% -------------
\usepackage{%
  amsthm,%
  amssymb,%
  mathrsfs,%
  mathtools,%
  gensymb,%
  braket,%
  mleftright,%
  nicefrac,%
  interval%
}
\intervalconfig{%
  soft open fences%
}

\mleftright

\newcommand*\bmmax{2}
\usepackage{bm}


% --------
% Diagrams
% --------

% Colours
\usepackage[usenames, svgnames, x11names, rgb]{xcolor}

% Graphics
\usepackage{graphicx}
\usepackage{grffile}

% TikZ & PGFPlots
\usepackage{pgfplots}

% Set up tikzexternalize
\usetikzlibrary{external}
\tikzexternalize
% \tikzexcmd is defined in the compilation call from the command line. See the Makefile.
\newif\iftikzex
\ifdefined\notikzex
  \tikzexfalse
\else
  \tikzextrue
\fi

\iftikzex
  \pgfplotsset{compat=1.18}

  \usetikzlibrary{
    calc,
    luamath,
    positioning,
    decorations.pathreplacing,
    backgrounds,
    arrows.meta,
    pgfplots.groupplots,
    pgfplots.patchplots,
    3d,
  }

  \usepgfplotslibrary[colormaps]

  \pgfplotscreateplotcyclelist{coloronly}{
    {red},
    {blue},
    {black!60!green},
    {black!20!orange},
    {black!30!blue},
    {green!30!brown},
    {blue!40!red},
    {IndianRed},
    {black!40!yellow},
    {Magenta4},
    {DodgerBlue4},
    {Maroon4},
    {Firebrick4},
    {Cyan4},
  }
\fi
\tikzexfalse

% Plot conditionals
\usepackage{xifthen}


% --------
% Captions
% --------
\usepackage{caption, subcaption}


% ------
% Tables
% ------
\usepackage{%
  booktabs,%
  array,%
  adjustbox,%
  makecell,%
  multirow,%
  bigdelim%
}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}m{#1}}

% -----
% Items
% -----
\usepackage[inline]{enumitem}


% --------
% Theorems
% --------
\theoremstyle{plain}
\newtheorem{proposition}{Proposition}
\theoremstyle{remark}
\newtheorem*{remark}{Remark}


% ----------
% Hyperlinks
% ----------
\usepackage[%
  hyperfootnotes=false,%
  hypertexnames=false,%
  hidelinks,%
]{hyperref}
\hypersetup{%
  bookmarksnumbered=true,%
  colorlinks=true,%
  citecolor=teal,%
  linkcolor=Blue4,%
}


% ------------
% Bibliography
% ------------
\usepackage{mciteplus}

% ---------
% Debugging
% ---------
%\listfiles
